Mathematical modelling of decision cycles in a competitive environment with neutral parties

Decision making is a human process that is a fundamental part of competition. As a realisation of decision making, Command and Control, or C2, has been studied in the literature for adversarial populations, yet these models do not explicitly capture competition. Our work here seeks to enrich such competition models by extending ecologically inspired population models to include decision dynamics through coupling with a nonlinear system of oscillators (the Kuramoto equation) to model the action-perception cycle in decision making. Through asymmetric competition models of increasing complexity, we highlight the importance of competitive agility and decision making processes necessary for a population to be successful.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
